GVE-LPA: Fast Label Propagation Algorithm (LPA) for Community Detection in Shared Memory Setting

Community detection is the problem of identifying natural divisions in networks. Efficient parallel algorithms for this purpose are crucial in various applications, particularly as datasets grow to substantial scales. This technical report presents an optimized parallel implementation of the Label Propagation Algorithm (LPA), a high speed community detection method, for shared memory multicore systems. On a server equipped with dual 16-core Intel Xeon Gold 6226R processors, our LPA, which we term as GVE-LPA, outperforms FLPA, igraph LPA, and NetworKit LPA by 139x, 97000x, and 40x respectively - achieving a processing rate of 1.4B edges/s on a 3.8B edge graph. In addition, GVE-LPA scales at a rate of 1.7x every doubling of threads.

==> src/fig-rak-speedup.tex <==
\begin{figure*}[hbtp]
  \centering
  \subfigure{
    \label{fig:rak-speedup--all}
    \includegraphics[width=0.98\linewidth]{out/rak-speedup.pdf}
  } \\[-2ex]
  \caption{Speedup of \textit{GVE-LPA} with respect to \textit{igraph}, \textit{FLPA}, and \textit{NetworKit} for each graph in the dataset.}
  \label{fig:rak-speedup}
\end{figure*}

